MMBench-Video: A Long-Form Multi-Shot Benchmark for Holistic Video Understanding

The advent of large vision-language models (LVLMs) has spurred research into their applications in multi-modal contexts, particularly in video understanding. Traditional VideoQA benchmarks, despite providing quantitative metrics, often fail to encompass the full spectrum of video content and inadequately assess models' temporal comprehension. To address these limitations, we introduce MMBench-Video, a quantitative benchmark designed to rigorously evaluate LVLMs' proficiency in video understanding. MMBench-Video incorporates lengthy videos from YouTube and employs free-form questions, mirroring practical use cases. The benchmark is meticulously crafted to probe the models' temporal reasoning skills, with all questions human-annotated according to a carefully constructed ability taxonomy. We employ GPT-4 for automated assessment, demonstrating superior accuracy and robustness over earlier LLM-based evaluations. Utilizing MMBench-Video, we have conducted comprehensive evaluations that include both proprietary and open-source LVLMs for images and videos. MMBench-Video stands as a valuable resource for the research community, facilitating improved evaluation of LVLMs and catalyzing progress in the field of video understanding. The evalutation code of MMBench-Video will be integrated into VLMEvalKit: https://github.com/open-compass/VLMEvalKit.

==> 99_supp_arxiv.tex <==
\appendix

\section{Additional Experiments}

\subsection{The Impact of Incorporating Speech over the entire MMBench-Video}

In the main paper, we report the quantitative results of speech improvement on the subset of videos with subtitles available from YouTube. 
In MMBench-Video, approximately half of videos do not include parseable video title tracks. 
In \cref{tab:vtt_augmented_whole}, 
we report the impact of incorporating speech information across the entire MMBench-Video dataset. 
Initially, we tested GPT-4o without visual input, and the results showed that even advanced models struggle to solve most problems using only question inputs. However, with subtitles, the model's ability to visualize content improves, boosting performance by 200\%. Further experiments with 8 and 16 frame inputs show that, even though only half of the VideoQAs include speech, the overall performance on the full benchmark remains significantly enhanced.
While only half of the VideoQAs are enhanced with speech, 
the overall performance improvement on the full benchmark remains significant. 
It is evident that the enhancement in reasoning capabilities surpasses that of perceptual abilities.
Speech typically conveys contextual information absent in static visual inputs,  
facilitating further reasoning by the VLM.
Meanwhile, improvements in coarse perception are minimal or remain largely unchanged 
(for GPT-4o-[16f]). 
This can be attributable to the fact that perception is predominantly reliant on visual inputs, and speech information does not significantly augment the model's performance in coarse perception.


% Compared to \cref{tab:vtt_augmented}, it is clear that the improvement in reasoning capability is more pronounced. This is likely because speech can convey contextual information not present in static visual inputs, aiding the model in further reasoning.
% whole 的 relation reasoning 比 subset都要高，异常现象，这个需要解释吗？
% 应该没有必要吧，就是不同的 video 集合

% Regarding perception, improvements in coarse perception are very limited or nearly unchanged. This may be due to the fact that perception relies more heavily on visual inputs, and speech information does not significantly enhance the model's coarse perception performance.
%perception上FP-C更在subset更显著，是不是可以说subtitle在cross instance的感知上有更大帮助。

\begin{table}[ht]
\small 
\centering
\resizebox{\textwidth}{!}{
\tablestyle{10pt}{1.3}
\begin{tabular}{lc|c|cccc|c|ccccc|c}
\shline 
\multirow{2}{*}{\bf Model} & \multirow{2}{*}{\bf \makecell{Subtitle}} & \multirow{2}{*}{\bf \makecell{Overall \\Mean}} & \multicolumn{5}{c}{{\cellcolor{maroon}}{\bf Perception}} &  \multicolumn{6}{c}{{\cellcolor{lightblue}}{\bf Reasoning}} \\ \scline{4-14}
& & & \textbf {CP} & \textbf {FP-S} & \textbf {FP-C} & \textbf {HL} & \textbf {Mean} & \textbf {LR} & \textbf {AR} & \textbf {RR} & \textbf {CSR} & \textbf {TR} & \textbf {Mean} \\ \shline
\multirow{2}{*}{GPT-4o} & \ding{56} &0.25 & 0.03 &	0.11 &	0.07 &	1.82 &	0.16 &	0.39 &	0.55 &	0.32 &	0.30&	0.55&	0.45\\
& \ding{52}	& 0.74	&0.60&	0.64&	0.50&	2.11&	0.67&	0.46&	0.98&	0.91&	0.44&	0.94&	0.83 \\ \shline
\multirow{2}{*}{GPT-4o-[8f]} & \ding{56} &1.62 & 1.82 &	1.59 &	1.43 &	1.95 &	1.63 &	1.33 &	1.89 &	1.60 &	1.60&	1.44&	1.57\\
& \ding{52}	& 1.79	&1.90&	1.82&	1.51&	1.82&	1.79&	1.57&	1.98&	1.81&	1.81&	1.71&	1.78 \\ \shline
\multirow{2}{*}{GPT-4o-[16f]} & \ding{56} &1.86&	2.03&	1.88&	1.67&	2.13&	1.89&	1.78&	1.95	&1.78	&1.90&	1.68&	1.80\\
& \ding{52} &1.96&	2.03&	2.00&	1.77&	1.89&	1.97&	1.87&	1.98&	1.92&	1.99	&1.84	&1.90\\ \shline
\end{tabular}
}
\vspace{2mm}
\caption{\textbf{GPT-4o's performance can be further improved by incorporating YouTube generated subtitles even under whole dataset.} 
% -[NV] indicates the model only take text information as input.
}
\label{tab:vtt_augmented_whole}
\vspace{-3mm}
\end{table}

% \subsection{Correlation between video duration and model performance}

% To explore the influence between video duration and model performance, we averaged the scores of the individual questions for each video as the score for the video, divided them into groups based on duration like \cref{fig:stat-duration}, and plotted a line graph.

% To investigate the relationship between video duration and model performance, we averaged the scores of individual questions for each video to obtain an overall score for the video. We then grouped these scores based on video duration, as shown in \cref{fig:stat-duration}, and plotted a line graph.

% \begin{figure*}
%     \centering
%     \includegraphics[width=0.5\linewidth]{figure/video_len_vs_score.png}
%     \caption{\textbf{As the video gets longer, the rating gets lower.} We use GPT-4o-[8f] data to make this chart.}
%     \label{fig:video_len_vs_score}
% \end{figure*}

% As shown in \cref{fig:video_len_vs_score}, it's obvious that video length has an overall negative correlation with model performance. That might because video time growth makes the number of sampled video frames sparser, and also makes it more difficult for the model to accurately answer the sudden increase in the number of questions that can be asked across time domains.

\subsection{Detailed Analysis of L-2 Capability}

Based on \cref{tab:main-results}, 
it is evident that hallucination is the most significant limitation in L-2 perceptual capabilities for all Video-LLMs, 
in contrast to the state-of-the-art proprietary LVLMs.
This indicates that existing Video-LLMs are unable to dismiss questions 
pertaining to videos when uncertain 
and are inclined to generate answers for questions regarding non-existent visual content.
% Additionally, the better performing features of Video-LLM L-2, such as fine-grained perception, relational reasoning, and attribute reasoning, appear to be more fundamental.

Regarding LVLMs, the number of frames significantly influences the performance of most L-2 capabilities in MMBench-Video. 
With an increase in the number of frames, the enhancement in perceptual capabilities becomes more pronounced than that in reasoning capabilities.
Owing to a more extensive training corpus and superior safety mechanisms, 
proprietary LVLMs exhibit superior performance in challenging capabilities such as logical reasoning, commonsense reasoning, and hallucination.

Interestingly, despite Idefics2-8B-[1f] utilizing a single image as input, 
it still outperforms all Video-LLMs in temporal reasoning tasks. 
This suggests that Video-LLMs are not effectively leveraging diverse temporal information, 
underscoring the necessity to enhance the diversity of instruction tuning data for these models.

% 1. 针对开源video-llm， 幻觉辨识能力整体较差，细粒度感知不如粗粒度感知。attribute /relation reasoning优于更困难的Logical reasoning和commonsense reasoning.
% 2.open-source lvlm, 除幻觉外的各方面L2 capabiliy 会随着 frame 数增多而提高，感知的增长幅度更大，temporal reasoning并不弱于video的模型
% 3. 开源lvlm的抗幻觉能力更强，csr,lr等较难的reasoning表现更好
% 4. 纵向对比，temporal reasoning即使是单帧的idefics2-8b仍旧优于多帧的所有Video-llm，说明video-llm利用temporal信息还不够，同时可能可以考虑注入更多的图文数据，及指令微调数据以提升csr和lr能力

\subsection{Model Performance across Video Time Length and Video Shots}

The length of the video and the number of shots are indeed key factors affecting model performance. Videos with fewer and shorter shots may perform better at lower frame counts, while longer or multi-shot videos require more visual content to fully leverage the model's capabilities.

\cref{fig:video_length} illustrates the trend of model scores in relation to shot count and video length. It is evident that the performance of GPT-4o, sampled at different frame rates, declines as video length increases, whereas the performance of open-source models such as InternVL-Chat-v1.5 and Video-LLaVA remains relatively stable. Compared to video length, model performance is more significantly influenced by the number of video shots. With over 50 shots in a video, the performance of GPT-4o drops to 75\% of its original score. This suggests that the model's performance is more closely tied to the number of shots than to video length, as the frequent shot transitions make it more challenging for the model to comprehend the video, resulting in lower scores.

\begin{figure*}
\centering
\includegraphics[width=.8\linewidth]{figure/length&shots.pdf}
% \vspace{-0.2em}
\caption{\textbf{Performance across varying video lengths and video shots}. We report the results of InternVL-Chat-V1.5-[1/8f], GPT-4o-[1/8f] and Video-LLaVA judged by GPT-4-Turbo (1106). 
}
\label{fig:video_length}
\vspace{-5mm}
\end{figure*}

\section{Additional Dataset Analysis}

In this section, we present more details about the MMBench-Video dataset: 
including the technique we adopted to filter temporal dispensable questions and 
some statistics on the linguistic characteristics of questions in MMBench-Video.
In \cref{fig:sample-video1,fig:sample-video2,fig:sample-video3}, 
we display a selection of samples from MMBench-Video, 
showcasing videos, images, questions, and reference answers for illustrative purposes.

% \paragraph{Video} The sample video provided is taken from the TV series \textit{Mr. Bean}. The video file can be found in the supplementary materials. \cref{fig:sample-video} shows an image obtained by sampling according to the 9-image method described in Section 4.3.

% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{figure/SpfvFl3p4is.png}
%     \caption{\textbf{Frames in the Sampled Video.}}
%     \label{fig:sample-video}
%     \vspace{-3mm}
% \end{figure*}

% \paragraph{Question-Answer Pairs} For the above video, we have annotated several QA pairs, listed in \cref{tab:sample_qa}.

% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{
% \tablestyle{5pt}{1.3}
% \begin{tabular}{@{}ccc@{}}
% \shline
% L-3 Capabilities & Question  & Answer   \\ \shline
% \begin{tabular}[c]{@{}c@{}}Function Reasoning\\ Object Recognition\end{tabular} & \begin{tabular}[c]{@{}c@{}}How does Mr.Bean steer when he was \\ sitting on top of the car?\end{tabular}                                 & He use a rope to steer.                                                                                            \\ \shline
% \begin{tabular}[c]{@{}c@{}}Function Reasoning\\ Object Recognition\end{tabular} & \begin{tabular}[c]{@{}c@{}}What does Mr. Bean use to operate the \\ brakes and gas pedal of his car?\end{tabular}                        & He uses a mop to do it.                                                                                            \\ \shline
% \begin{tabular}[c]{@{}c@{}}OCR\\ Object Recognition\end{tabular}                & What occurs to Mr. Bean at the end?                                                                                                      & \begin{tabular}[c]{@{}c@{}}His car collides with a van \\ loaded with beddings.\end{tabular}                       \\ \shline
% Video Emotion                                                                   & \begin{tabular}[c]{@{}c@{}}What might the people sitting outside the store \\ feel after seeing the guy's sorta magic show?\end{tabular} & \begin{tabular}[c]{@{}c@{}}They might feel weird and \\ get frightened.\end{tabular}                               \\ \shline
% Video Style                                                                     & \begin{tabular}[c]{@{}c@{}}This video is more likely to be \\ filmed in 1990s or 2020s?\end{tabular}                                     & \begin{tabular}[c]{@{}c@{}}The video is more likely filmed in \\ 1990s due to the bad visual quality.\end{tabular} \\ \shline
% \end{tabular}}
% \caption{\textbf{Quetion-Answer Pairs for the Sample Video.}}
% \label{tab:sample_qa}
% \vspace{-3mm}
% \end{table*}


\subsection{Temporal Dispensable Data Filtering with LVLM}

To ensure that the majority of questions in MMBench-Video are temporally indispensable,
we implement an LVLM-based filtering process and subsequently conduct manual verification.
Specifically, we employ GPT-4v, one of the most potent LVLMs, 
to filter out questions exhibiting high temporal irrelevance.
Utilizing four distinct random seeds, 
we sample a single random frame as visual input for each individual VideoQA instance and conduct the inference four times. 
Subsequently, we utilize GPT-4 to evaluate the responses and compute the average score for each question.
Questions with an average score of 2.5 or higher across the four responses were excluded from the benchmark. 
Based on this approach, we removed a total of 246 temporally dispensable questions from the dataset.


% 这部分正文说过了
% Since most Video-LLMs and advanced LVLMs lack temporal localization capabilities, timestamp information is redundant in the question. One of our authors deleted or revised questions with specific timestamps for this reason. For example, for a 3-minute video, the question "At around 13s in the video, what state might the water in the pot be in before adding pasta to the pot?" was changed to "At the beginning of the video, what state might the water in the pot be in before adding pasta to the pot?".

% GPT-4 then provided scoring judgements based on GPT-4v responses. We calculated the average score for each question, and those with an average score above 2.5 out of four responses were deleted. Using this method, we removed a total of 246 static questions, as they yielded highly similar answers regardless of the input content.


% The average score for each question can be calculated, and questions with an average of four responses above 2.5 will be deleted. Under this principal, a total of 246 static questions have been deleted since they give highly similar answers even if the input content is completely different.

\subsection{Question Type Analysis}
\begin{figure*}
\centering
\includegraphics[width=.8\linewidth]{figure/q_type.pdf}
% \vspace{-0.2em}
\caption{\textbf{Comparison of question type distribution with MSVD and MSRVTT.} MMBench-Video encompasses a more extensive assortment of question types and exhibits a distribution that is more equitably balanced among these various categories. 
}
\label{fig:question}
\vspace{-5mm}
\end{figure*}



Given that the majority of existing Video-QA benchmarks are characterized by a limited range of question types, 
which fail to adequately represent the diverse spectrum of human conversations, 
the question set within MMBench-Video has been meticulously curated to encompass a wide variety of categories. 
We visualize the comparison of the question type distribution between MMBench-Video and other popular benchmarks in \cref{fig:question}. 
In addition to the conventional question archetypes,
namely \textit{‘what’, ‘who’, ‘how’, ‘when’, and ‘where’},
MMBench-Video extends its corpus to include additional interrogatives such as 
\textit{‘why’, ‘which’, ‘is / are’, and ‘does / do’}. 
The expansion diversifies the dataset and closely aligns with the style of natural human dialogues. 
Meanwhile, the question type distribution within MSVD or MSRVTT exhibits a significant skew. 
The category of `what' predominates, comprising over 60\% of the questions, 
in stark contrast to the significantly underrepresented categories such as ‘when’ and ‘where’, 
totaling a mere 1\%. 
Nevertheless, the question type distribution within MMBench-Video has been deliberately engineered to achieve a greater equilibrium. 
While the `what’ category maintains its status as the most prevalent, the remaining question types are evenly distributed across various interrogative forms.

\begin{figure*}
    \centering
    \includegraphics[width=.95\linewidth]{samples/Games.pdf}
    \\
    \vspace{2mm}
    \includegraphics[width=.95\linewidth]{samples/Sports.pdf}
    \\
    \vspace{2mm}
    \includegraphics[width=.95\linewidth]{samples/Advertisement.pdf}
    \caption{\textbf{Visualization of Samples in MMBench-Video.} Part 1 out of 3. }
    \label{fig:sample-video1}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{samples/News.pdf}
    \\
    \vspace{3mm}
    \includegraphics[width=\linewidth]{samples/Computer.pdf}
    \caption{\textbf{Visualization of Samples in MMBench-Video.} Part 2 out of 3. }
    \label{fig:sample-video2}
\end{figure*}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{samples/Food.pdf}
    \\
    \vspace{3mm}
    \includegraphics[width=\linewidth]{samples/Knowledge.pdf}
    \caption{\textbf{Visualization of Samples in MMBench-Video.} Part 3 out of 3. }
    \label{fig:sample-video3}
\end{figure*}

\section{Prompts Adopted in MMBench-Video}

In Sec. 3.1, we outline the LLM-involved evaluation paradigm we employ, 
utilizing GPT-4 for scoring. 
The evaluation is conducted through prompts configured with a 3-grade marking (0, 1, 2, 3). 
In this section, we elaborate on the specific prompts utilized in the evaluation process.

\subsection{System Prompt for GPT-based Evaluation} 

\texttt{\small As an AI assistant, your task is to evaluate a candidate answer in comparison to a given correct answer. The question itself, the correct 'groundtruth' answer, and the candidate answer will be provided to you. Your assessment should range from 0 to 3, based solely on the semantic similarity between the groundtruth and the candidate answer, disregarding any grammatical differences. A rating of 0 suggests no similarity, implying the candidate answer is entirely incorrect. A rating of 1 suggests low similarity, meaning the candidate answer is largely incorrect. A rating of 2 suggests high similarity, meaning the candidate answer is largely correct. Lastly, a rating of 3 indicates complete similarity, which means the candidate answer is entirely correct. Your response should be a single integer from 0, 1, 2, or 3.\\
Question: [QUESTION]\\
Groundtruth answer: [ANNOTATED ANSWER]\\
Candidate answer: [CANDIDATE ANSWER]\\
Your response: }

\subsection{System Prompt for the Inference of LVLMs with Multi-Frame Inputs} 

\texttt{\small You will be provided with [FRAME NUM] separate frames uniformly sampled from a video, the frames are provided in chronological order of the video. \\
Please analyze these images and provide the answer / answers to the following question / questions about the video content.\\
If multiple questions are provided (with indices I1, I2, I3, ...), you should organize your answers in the following json format:\\
$\{$\\
\hspace*{5mm} `I1': 'Answer to Question I1', \\
\hspace*{5mm} `I2': 'Answer to Question I2', \\
\hspace*{5mm} ...\\
$\}$\\
Otherwise, please directly reply with your response to the only question. \\
Even if the information in these separate frames is not enough to give an answer, PLEASE TRY YOUR BEST TO GUESS A CLEAR OR VAGUE ANSWER WHICH YOU THINK WOULD BE THE MOST POSSIBLE ONE BASED ON THE QUESTION.\\
Minimize negative responses such as `not possible to determine'. STIMULATE YOUR POTENTIAL AND IMAGINATION!\\}

\subsection{Input Prompt Template for the Inference of LVLMs with Multi-Frame Inputs}

\texttt{\small [System Prompt] \\ 
\quad [Subtitle (Optional): \{ \\
\hspace*{5mm} `t0' - `t1': subtitle 1, \\
\hspace*{5mm} `t1' - `t2': subtitle 2, \\
\hspace*{5mm} ...... \\
\}]\\
\quad [Multi-Frame Inputs] \\
\quad [Question Set: \{ \\
\hspace*{5mm} `index 1': question 1 for this video, \\
\hspace*{5mm} `index 2': question 2 for this video, \\
\hspace*{5mm} ...... \\
\}]}

\section{Limitations and Broader Impacts}
\label{sec:impacts}

\textbf{Limitations. }
In this study, we introduce MMBench-Video,
a novel long-form multi-shot VideoQA benchmark,
and perform a comprehensive evaluation based on this benchmark. 
In light of budget constraints, 
our evaluation is focused on a curated selection of representative open-source and proprietary VLMs, 
which may not encompass all those most recent high-performing models. 
GPT-4 is adopted as a more advanced judge model for scoring the responses, 
while further experiments should be conducted in the future to study the feasibility of 
using state-of-the-art open-source LLMs as the judge.
Taking into account the limited capabilities of existing Video-LLMs,
we currently set the upper duration limit of videos to 6 minutes,
refraining from scaling to tens of minutes or hours.
The evaluation results indicate that,
even with relatively modest video durations, 
MMBench-Video presents a significant challenge to existing Video-LLMs.

\textbf{Broader Impacts. }
As an evaluation benchmark, 
MMBench-Video offers detailed insights into the fine-grained capabilities of diverse vision-language models (VLMs) in the domain of video understanding, 
providing valuable insights for future model optimization. 
The new benchmark exhibits enhanced quality and enriched diversity, and employs a more precise scoring strategy, 
which collectively contribute to comprehensive and reliable evaluation outcomes.
Leveraging MMBench-Video and other Image VQA benchmarks, 
we conduct a comprehensive evaluation of existing video-LLMs,
revealing their limited capabilities in both spatial and temporal understanding. 
Additionally, MMBench-Video, being a small-scale benchmark, 
may not encompass every video topic and fine-grained capability. 
There is a risk that MMBench-Video may not adequately reflect the video understanding capabilities of VLMs in specific tasks or scenarios. 
We encourage users to carefully consider the intended use cases of VLMs when utilizing MMBench-Video for evaluation.


==> mmstyle.tex <==
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{xspace}

% common abbreviations

\providecommand{\eg}{\textit{e.g.}\@\xspace}
\providecommand{\ie}{\textit{i.e.}\@\xspace}
\providecommand{\wrt}{\textit{w.r.t.}\@\xspace}
\providecommand{\etal}{\textit{et al}\@\xspace}

% for development

\newcommand{\miss}[1]{\textcolor{red}{#1}}
\newcommand{\misscite}{\textcolor{red}{[C]}}
\newcommand{\missref}{\textcolor{red}{[R]}}
\newcommand{\needcheck}[1]{\textcolor{red}{#1}}


% useful operators

\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}


% v? vectors:

\newcommand{\va}{\mathbf{a}}
\newcommand{\vb}{\mathbf{b}}
\newcommand{\vc}{\mathbf{c}}
\newcommand{\vd}{\mathbf{d}}
\newcommand{\ve}{\mathbf{e}}
\newcommand{\vf}{\mathbf{f}}
\newcommand{\vg}{\mathbf{g}}
\newcommand{\vh}{\mathbf{h}}
\newcommand{\vi}{\mathbf{i}}
\newcommand{\vj}{\mathbf{j}}
\newcommand{\vk}{\mathbf{k}}
\newcommand{\vl}{\mathbf{l}}
\newcommand{\vm}{\mathbf{m}}
\newcommand{\vn}{\mathbf{n}}
\newcommand{\vo}{\mathbf{o}}
\newcommand{\vp}{\mathbf{p}}
\newcommand{\vq}{\mathbf{q}}
\newcommand{\vr}{\mathbf{r}}
%\newcommand{\vs}{\mathbf{s}}
\newcommand{\vt}{\mathbf{t}}
\newcommand{\vu}{\mathbf{u}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\vw}{\mathbf{w}}
\newcommand{\vx}{\mathbf{x}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vz}{\mathbf{z}}

\newcommand{\vone}{\mathbf{1}}
\newcommand{\vzero}{\mathbf{0}}

\newcommand{\valpha}   {\boldsymbol{\alpha}}
\newcommand{\vbeta}    {\boldsymbol{\beta}}
\newcommand{\vgamma}   {\boldsymbol{\gamma}}
\newcommand{\vdelta}   {\boldsymbol{\delta}}
\newcommand{\vepsilon} {\boldsymbol{\epsilon}}
\newcommand{\vzeta}    {\boldsymbol{\zeta}}
\newcommand{\veta}     {\boldsymbol{\eta}}
\newcommand{\vtheta}   {\boldsymbol{\theta}}
\newcommand{\viota}    {\boldsymbol{\iota}}
\newcommand{\vkappa}   {\boldsymbol{\kappa}}
\newcommand{\vlambda}  {\boldsymbol{\lambda}}
\newcommand{\vmu}      {\boldsymbol{\mu}}
\newcommand{\vnu}      {\boldsymbol{\nu}}
\newcommand{\vxi}      {\boldsymbol{\xi}}
\newcommand{\vpi}      {\boldsymbol{\pi}}
\newcommand{\vrho}     {\boldsymbol{\rho}}
\newcommand{\vsigma}   {\boldsymbol{\sigma}}
\newcommand{\vtau}     {\boldsymbol{\tau}}
\newcommand{\vupsilon} {\boldsymbol{\upsilon}}
\newcommand{\vphi}     {\boldsymbol{\phi}}
\newcommand{\vchi}     {\boldsymbol{\chi}}
\newcommand{\vpsi}     {\boldsymbol{\psi}}
\newcommand{\vomega}   {\boldsymbol{\omega}}


% m? matrices:

\newcommand{\mA}{\mathbf{A}}
\newcommand{\mB}{\mathbf{B}}
\newcommand{\mC}{\mathbf{C}}
\newcommand{\mD}{\mathbf{D}}
\newcommand{\mE}{\mathbf{E}}
\newcommand{\mF}{\mathbf{F}}
\newcommand{\mG}{\mathbf{G}}
\newcommand{\mH}{\mathbf{H}}
\newcommand{\mI}{\mathbf{I}}
\newcommand{\mJ}{\mathbf{J}}
\newcommand{\mK}{\mathbf{K}}
\newcommand{\mL}{\mathbf{L}}
\newcommand{\mM}{\mathbf{M}}
\newcommand{\mN}{\mathbf{N}}
\newcommand{\mO}{\mathbf{O}}
\newcommand{\mP}{\mathbf{P}}
\newcommand{\mQ}{\mathbf{Q}}
\newcommand{\mR}{\mathbf{R}}
\newcommand{\mS}{\mathbf{S}}
\newcommand{\mT}{\mathbf{T}}
\newcommand{\mU}{\mathbf{U}}
\newcommand{\mV}{\mathbf{V}}
\newcommand{\mW}{\mathbf{W}}
\newcommand{\mX}{\mathbf{X}}
\newcommand{\mY}{\mathbf{Y}}
\newcommand{\mZ}{\mathbf{Z}}

\newcommand{\mGamma}{\boldsymbol{\Gamma}}
\newcommand{\mDelta}{\boldsymbol{\Delta}}
\newcommand{\mTheta}{\boldsymbol{\Theta}}
\newcommand{\mLambda}{\boldsymbol{\Lambda}}
\newcommand{\mXi}{\boldsymbol{\Xi}}
\newcommand{\mPi}{\boldsymbol{\Pi}}
\newcommand{\mSigma}{\boldsymbol{\Sigma}}
\newcommand{\mUpsilon}{\boldsymbol{\Upsilon}}
\newcommand{\mPhi}{\boldsymbol{\Phi}}
\newcommand{\mPsi}{\boldsymbol{\Psi}}
\newcommand{\mOmega}{\boldsymbol{\Omega}}


% c? calligraphic letters

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}


% blackboard bold

\newcommand{\Abb}{\mathbb{A}}

\newcommand{\Cbb}{\mathbb{C}}
\newcommand{\Dbb}{\mathbb{D}}
\newcommand{\Ebb}{\mathbb{E}}
\newcommand{\Fbb}{\mathbb{F}}
\newcommand{\Gbb}{\mathbb{G}}
\newcommand{\Hbb}{\mathbb{H}}
\newcommand{\Ibb}{\mathbb{I}}
\newcommand{\Jbb}{\mathbb{J}}
\newcommand{\Kbb}{\mathbb{K}}
\newcommand{\Lbb}{\mathbb{L}}
\newcommand{\Mbb}{\mathbb{M}}
\newcommand{\Nbb}{\mathbb{N}}
\newcommand{\Obb}{\mathbb{O}}
\newcommand{\Pbb}{\mathbb{P}}
\newcommand{\Qbb}{\mathbb{Q}}
\newcommand{\Rbb}{\mathbb{R}}
\newcommand{\Sbb}{\mathbb{S}}
\newcommand{\Tbb}{\mathbb{T}}
\newcommand{\Ubb}{\mathbb{U}}
\newcommand{\Vbb}{\mathbb{V}}
\newcommand{\Wbb}{\mathbb{W}}
\newcommand{\Xbb}{\mathbb{X}}
\newcommand{\Ybb}{\mathbb{Y}}
\newcommand{\Zbb}{\mathbb{Z}}


==> table/human_align_figure.tex <==
% \resizebox{\textwidth}{!}{
\begin{figure*}[t]
\centering
\begin{subfigure}{0.45\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/video_llava1.pdf}
\caption{Results of Video-LLaVA.}
\end{subfigure}
\hspace{1em}
\begin{subfigure}{0.45\textwidth}
\centering
\includegraphics[width=\textwidth]{figure/gpt4o1.pdf}
\caption{Results of GPT-4o.}
\end{subfigure}
\caption{\textbf{Rating distribution of different judge models. } 
We report the results of Video-LLaVA and GPT-4o respectively judged by GPT-3.5-Turbo (1106) and GPT-4-Turbo (1106). }
\label{fig:rating_distribution}
\vspace{-4mm}
\end{figure*}
% }

==> table/result.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}


\begin{tabular}{@{}ccccccccccccc@{}}
\toprule
mode                      & model                   & Average & \begin{tabular}[c]{@{}c@{}}Average \\ (w/o HL)\end{tabular} & CP   & FP{[}S{]} & FP{[}C{]} & LR   & AR   & RR   & CSR  & TR   & HL   \\ \midrule
\multirow{6}{*}{video}    & videochat               & 1.05    & 0.90                                                        & 1.19 & 0.86      & 0.79      & 0.44 & 1.05 & 1.20 & 0.69 & 1.03 & 2.21 \\
                          & video-chatgpt           & 0.75    & 0.75                                                        & 0.79 & 0.71      & 0.67      & 0.53 & 1.01 & 1.01 & 0.47 & 0.82 & 0.74 \\
                          & otter                   & 0.87    & 0.77                                                        & 0.94 & 0.80      & 0.72      & 0.49 & 0.90 & 0.91 & 0.60 & 0.79 & 1.67 \\
                          & llama-adapter           & 0.73    & 0.79                                                        & 0.72 & 0.71      & 0.80      & 0.63 & 0.70 & 1.20 & 0.56 & 1.02 & 0.28 \\
                          & mplug-owl               & 0.97    & 1.07                                                        & 1.35 & 1.00      & 0.82      & 0.68 & 1.29 & 1.42 & 0.89 & 1.12 & 0.17 \\
                          & moviechat               & 0.44    & 0.43                                                        & 0.97 & 0.56      & 0.41      & 0.11 & 0.40 & 0.61 & 0.18 & 0.24 & 0.46 \\ \midrule
\multirow{6}{*}{9 images} & videochat-image         & 1.07    & 0.97                                                        & 1.16 & 0.93      & 0.93      & 0.45 & 1.19 & 1.43 & 0.73 & 0.94 & 1.88 \\
                          & otter-image             & 0.85    & 0.82                                                        & 1.00 & 0.82      & 0.75      & 0.38 & 0.96 & 0.99 & 0.93 & 0.71 & 1.10 \\
                          & InternLM-XComposer(7B)  & 0.76    & 0.81                                                        & 1.13 & 0.78      & 0.67      & 0.47 & 1.05 & 1.04 & 0.62 & 0.70 & 0.40 \\
                          & Qwen-VL-Chat(7B)        & 1.00    & 0.97                                                        & 1.35 & 1.02      & 0.83      & 0.61 & 1.14 & 1.13 & 0.84 & 0.85 & 1.26 \\
                          & Idefics\_9B\_Instruct   & 0.90    & 0.95                                                        & 1.20 & 0.87      & 0.78      & 0.44 & 1.14 & 1.45 & 0.91 & 0.81 & 0.49 \\
                          & LLaVA-v1.5-13B          & 0.62    & 0.68                                                        & 0.90 & 0.72      & 0.66      & 0.42 & 0.65 & 0.96 & 0.53 & 0.57 & 0.15 \\ \midrule
\multirow{5}{*}{1 image}  & videochat-image         & 1.03    & 0.90                                                        & 1.14 & 0.85      & 0.77      & 0.50 & 1.01 & 1.15 & 0.70 & 1.11 & 2.06 \\
                          & otter-image             & 0.77    & 0.77                                                        & 0.98 & 0.79      & 0.66      & 0.46 & 0.89 & 0.91 & 0.71 & 0.76 & 0.76 \\
                          & InternLM-XComposer (7B) & 0.72    & 0.76                                                        & 1.05 & 0.82      & 0.55      & 0.47 & 0.86 & 0.99 & 0.59 & 0.71 & 0.45 \\
                          & Qwen-VL-Chat (7B)       & 0.91    & 0.84                                                        & 1.12 & 0.83      & 0.53      & 0.52 & 1.01 & 0.97 & 0.83 & 0.90 & 1.47 \\
                          & Idefics\_9B\_Instruct   & 0.96    & 1.02                                                        & 1.17 & 0.99      & 0.88      & 0.68 & 1.09 & 1.46 & 0.86 & 1.06 & 0.49 \\ \midrule
text                      & gpt4                    & 0.84    & 0.63                                                        & 0.19 & 0.25      & 0.29      & 0.59 & 0.88 & 1.05 & 0.58 & 1.22 & 2.50 \\ \midrule
text+subtitle             & gpt4                    & 0.70    & 0.47                                                        & 0.46 & 0.42      & 0.34      & 0.25 & 0.54 & 0.85 & 0.53 & 0.40 & 2.55 \\ \bottomrule
\end{tabular}


\caption{\textbf{Evalutaion Result on MMBench-Video.} CP, FP[S], FP[C] stands for Perception tasks, LR, AR, RR, CSR, TR stand for Reasoning tasks. HL stands for the Hallucination test. All scores are on a 3-point scale. The higher HL score, the less hallucination the model has.}
\label{tab:mmbench-video-result}
\end{table*}
